Estimating the Impact of foregrounds on the Future Detection of Rayleigh scattering

Rayleigh scattering of the cosmic microwave background (CMB) by neutral hydrogen shortly after recombination leaves frequency-dependent imprints on intensity and polarization fluctuations. High signal-to-noise observations of CMB Rayleigh scattering would provide additional insight into the physics of recombination, including greater constraining power for parameters like the primordial helium fraction, the light relic density, and the sum of neutrino masses. However, such a measurement of CMB Rayleigh scattering is challenging due to the presence of astrophysical foregrounds, which are more intense at the high frequencies, where the effects of Rayleigh scattering are most prominent. Here we forecast the detectability of CMB Rayleigh scattering including foreground removal using blind internal linear combination methods for a set of near-future surveys. We show that atmospheric effects for ground-based observatories and astrophysical foregrounds pose a significant hindrance to detecting CMB Rayleigh scattering with experiments planned for this decade, though a high-significance measurement should be possible with a future CMB satellite.

==> journals.tex <==
% Journal definitions
\def\aap{A\&A}
\def\aaps{A\&AS}
\def\aj{AJ}
\def\apj{ApJ}
\def\apjl{ApJL}
\def\apjs{ApJS}
\def\apss{APSS}
\def\araa{ARAA}
\def\jcap{JCAP}
\def\mnras{MNRAS}
\def\na{New Astronomy}
\def\nat{Nature}
\def\pasp{PASP}
\def\physrep{Phys. Rep.}
\def\prd{Phys. Rev. D}
\def\etal{et al.}
\def\pasj{PASJ}
\def\prl{Phys. Rev. D Letters}
\def\baas{BAAS}
\def\procspie{SPIE}
